The size-Ramsey number of cubic graphs

We show that the size-Ramsey number of any cubic graph with $n$ vertices is $O(n^{8/5})$, improving a bound of $n^{5/3 + o(1)}$ due to Kohayakawa, R\"{o}dl, Schacht, and Szemer\'{e}di. The heart of the argument is to show that there is a constant $C$ such that a random graph with $C n$ vertices where every edge is chosen independently with probability $p \geq C n^{-2/5}$ is with high probability Ramsey for any cubic graph with $n$ vertices. This latter result is best possible up to the constant.

==> embedding.tex <==
%!TEX root = size_ramsey.tex
\section{Stable embeddings and the Embedding Lemma}
\label{sec:embedding-lemma}

In this section we prove the most important ingredient of our proof
strategy---the Embedding Lemma. Before we state the lemma, it is convenient to
introduce a couple of definitions. First is that of a candidate set, mentioned
informally in Section~\ref{sec:strategy-trees}.

\begin{definition}
  Let $G$, $H$ be graphs, $S \subseteq V(H)$ a subset, and $\phi \colon S \to
  V(G)$ a function. For a vertex $v \in V(H) \setminus S$, we let $\CS_G^\phi(v,
  S)$ denote the {\em candidate set} for $v$ in $G$ defined as
  \[
    \CS_G^\phi(v, S) := \hat N_G \big( \phi(N_H(v, S)) \big) \setminus \phi(S).
  \]
\end{definition}

We write $\CS_G^\phi(v)$ if $S$ is an empty set. In plain words, $\CS_G^\phi(v,
S)$ is just the set of `free' vertices (not taken by the mapping of $S$) among
the common neighbourhood of the images of the vertices in $N_H(v)$ under $\phi$.
For example, if $\phi$ was a proper embedding, then mapping $v$ into any vertex
of $\CS_G^\phi(v, S)$ extends the embedding of $H[S]$ (by preserving edge
relations) into that of $H[S \cup \{v\}]$. For an illustration, see
Figure~\ref{fig:candidate-set}.

\begin{figure}[!htbp]
  \centering
  \includegraphics[scale=0.8]{figures/candidate-set-2}
  \caption{An example of a candidate set $\CS_G^\phi(v, S)$ for the vertex $v$
  given in red. The part of its neighbourhood $N_H(v, S)$ embedded before it and
  the vertices it is mapped to is given in blue. The embedding $\phi$ is given
  with green arrows.}
  \label{fig:candidate-set}
\end{figure}

The following notion plays a central role in the embedding process. As our
strategy revolves around embedding the graph $H$ into (lower-)regular pairs in
$\Gnp$ given by the sparse regularity lemma
(Theorem~\ref{thm:sparse-regularity-lemma}), there are a plethora of
technicalities to take care of. We define {\em stable mappings} in order to
gather all of them under one name.

\begin{definition}[$(\beps, p, c)$-stable mapping]
  Let $G, H$ be graphs with $\Delta(H) \leq \Delta$ and $V(G) = V_1 \cup \dotsb
  \cup V_{\Delta^2 + 1}$, with $|V_i| = n$ for all $i \in [\Delta^2 + 1]$. Given
  $p \in (0, 1)$, a vector $\beps = (\eps_0, \eps_1, \ldots, \eps_{2\Delta -
  1})$, a function $c \colon V(H) \to [\Delta^2 + 1]$, and a subset $S \subseteq
  V(H)$, we say that a function $\phi \colon S \to V(G)$ is an $(\beps, p,
  c)$-{\em stable mapping} if
  \begin{enumerate}[label=(S\arabic*), font=\itshape, leftmargin=3em]
    \item\label{stable-colour-class} $\phi(v) \in V_{c(v)}$ for all $v \in S$,
    \item\label{stable-embedding-edges} $\phi(u)\phi(v) \in G$ for every edge
      $uv \in H[S]$,
    \item\label{stable-large-neighbourhoods} $|\CS_G^\phi(v) \cap V_{c(v)}| \geq
      n(p/2)^{d_v}$, for all $v \in V(H) \setminus S$, where $d_v = \deg_H(v,
      S)$, and
    \item\label{stable-regularity-inheritance} $\big( \CS_G^\phi(u) \cap
      V_{c(u)}, \CS_G^\phi(v) \cap V_{c(v)} \big)$ is $(\eps_{d_{uv}},
      p)$-lower-regular for all $uv\in H[V(H) \setminus S]$, where $d_{uv} =
      \deg_H(u, S) + \deg_H(v, S)$.
  \end{enumerate}
\end{definition}

We provide a bit of explanation for the definition. The first two properties are
straightforward: \ref{stable-colour-class} makes the embedding of $H$
`canonical' where the `canonical' part is given by a function $c$, which is
usually taken to be a proper colouring of the square $H^2$ of the graph $H$,
while \ref{stable-embedding-edges} makes sure that $\phi$ actually produces an
embedding, i.e.\ that the edge relations are preserved. The third,
\ref{stable-large-neighbourhoods}, maintains the size of candidate sets for all
the remaining vertices, and perhaps the most crucial one
\ref{stable-regularity-inheritance} ensures that all the candidate sets of
future vertices are regular amongst themselves. These last two properties is
what allows some partial embedding of $H$ to be `extended' into a larger one.

% \begin{lemma}[Embedding Lemma]\label{lem:magic-embedding-lemma} For all
% $\alpha, \xi \in (0, 1]$, there exist positive constants $\beta(\alpha, \xi)$,
% $\eps(\alpha, \xi)$, and $C(\alpha, \xi)$ such that w.h.p.\ a random graph
% $\Gamma \sim \Gnp$ satisfies the following, provided that $p \geq Cn^{-2/5}$.

%   Let $H$ be a graph with $v(H) \leq \beta n$ and $\Delta(H) \leq \Delta$, for
%   some $\Delta \in \N$. Let $G \subseteq \Gamma$ belong to $\cG(K_{2\Delta^2 +
%   1}, \tilde n, \eps, \alpha p)$, where $\tilde n \geq \xi n$, and let $c \colon
%   V(H) \to [2\Delta^2 + 1]$ be an injective function. Let $\varnothing = S_0
%   \subset S_1 \subset \dotsb \subset S_t = V(H)$ be a chain of subsets for some
%   $t \geq 1$, such that
%   % Let $G \subseteq \Gamma$ belong to $\cG(F, \tilde n, \alpha, \eps, p)$, where
%   % $v(F) \geq 2$ and $\tilde n \geq \xi n$, let $H$ be a graph with $v(H) \leq
%   % \beta n$, and $c \colon V(H) \to V(F)$ an injective function. Let $\varnothing
%   % = S_0 \subset S_1 \subset \ldots \subset S_t = V(H)$ be a chain of subsets,
%   % for some $t \geq 1$, such that
%   \[
%     \deg_H(v, S_{i - 1}) \leq 1 \qquad \text{ for all $v \in S_i \setminus S_{i -
%     1}$ and $i \in [t]$}.
%   \]
%   Let $\beps = (\eps_0, \ldots, \eps_{2\Delta - 1})$, where $0 < \eps_i \leq
%   \eps$, for all $i \in [2\Delta - 1]$. Suppose that for every $i \in [t]$, every
%   $(\beps, \alpha p, c)$-stable embedding $\psi \colon S_{i - 1} \to V(G)$ can
%   be extended to an $(\beps, \alpha p, c)$-stable embedding $\phi \colon S_i \to
%   V(G)$ which, for every choice of subsets
%   \[
%     W_v \subseteq \CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}
%   \]
%   satisfying $|W_v| \geq (\xi/8)\tilde n(\alpha p/2)^{\deg_H(v, S_{i - 1})}$,
%   for all $v \in S_i \setminus S_{i - 1}$, maps $v$ to some $\phi(v) \in W_v$.
%   Then $G$ contains a copy of $H$.
% \end{lemma}

With those at hand, we are ready to give the full, somewhat technical and
tricky, statement. Some of the reasons for this are highlighted in the
discussion at the beginning of Section~\ref{sec:strategy-trees}.

\begin{lemma}[Embedding Lemma]\label{lem:magic-embedding-lemma}
  For all $\alpha, \mu, \xi > 0$, there exist positive constants $\beta(\alpha,
  \mu)$ and $C(\alpha, \mu)$ such that w.h.p.\ a random graph $\Gamma \sim \Gnp$
  satisfies the following, provided that $p \geq Cn^{-2/5}$.

  Let $H$ be a graph with $v(H) \leq \beta n$ and $\Delta(H) \leq 3$. Let $G
  \subseteq \Gamma$ be a graph with vertex set $V_1 \cup \dotsb \cup V_{10}$,
  where $|V_1| = \dotsb = |V_{10}| = \mu n$, and let $c \colon V(H) \to [10]$ be
  a function. Let $\varnothing = S_0 \subset S_1 \subset \dotsb \subset S_t =
  V(H)$ be a chain of subsets for some $t \geq 1$, such that
  \[
    \deg_H(v, S_{i - 1}) \leq 1 \qquad \text{ for all $v \in S_i \setminus S_{i
    - 1}$ and $i \in [t]$}.
  \]
  Let $\beps = (\eps_0, \eps_1, \dotsc, \eps_5)$, where $\eps_i \in (0, 1)$.
  Suppose that for every $i \in [t]$, every $(\beps, \alpha p, c)$-stable
  embedding $\psi \colon S_{i - 1} \to V(G)$ for which there exist subsets
  \[
    W_v \subseteq \CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}
  \]
  satisfying $|W_v| \geq \xi|V_{c(v)}|(\alpha p/2)^{\deg_H(v, S_{i - 1})}$ for
  all $v \in S_i \setminus S_{i - 1}$, can be extended to an $(\beps, \alpha p,
  c)$-stable embedding $\phi \colon S_i \to V(G)$ which maps $v$ to some
  $\phi(v) \in W_v$. Then $G$ contains a copy of $H$.
\end{lemma}

At the first glance the conclusion seems vacuous---if there is a stable
embedding of an empty set with sets $W_v$ as required (which is trivial) which
can be extended into a stable embedding of $S_1$ which can then be further
extended into a stable embedding of $S_2$, etc., then we can embed the whole
graph $H$. The intricacy lies in the fact that the mappings $\psi$ and $\phi$
need not control how much `space' they leave for the rest of the graph $H$. For
example, if $\psi$ leaves no space for some $v \in S_i \setminus S_{i - 1}$ by
having $\CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)} = \varnothing$, the rest of the
statement is empty, as in such an embedding the required sets $W_v$ do not exist
and consequently it cannot be extended into a stable embedding $\phi$. This is
where the true crux of the lemma resides. It ensures that, if we could have the
sets $\CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}$ sufficiently large throughout,
that is for all $i \in [t]$ and $S_i$, and then choose the sets $W_v$ in a
suitable manner, the stable embeddings actually produce a real copy of $H$ in
$G$ at the end.

Actually, the more cumbersome part of this lemma does not come from showing its
{\em conclusion} holds but from checking its {\em conditions} hold once we are
to apply it. Namely, we need that {\em every} stable embedding of $S_i$ can be
extended into a stable embedding of $S_{i + 1}$ for {\em all} $i \in [t]$ which
in addition maps vertices into prescribed subsets. The interesting bit is that
the lemma does not care about how the embeddings are given as long as they are
stable.

Lastly, we remark that, in general, the statement can be slightly strengthened.
For one, the maximum degree of $H$ need only be bounded, e.g.\ $\Delta(H) \leq
\Delta$ for some fixed $\Delta \in \N$. Perhaps more importantly, the condition
$\deg_H(v, S_{i - 1}) \leq 1$ can further be relaxed into $\deg_H(v, S_{i - 1})
\leq \Delta - 1$ for as long as $p \gg n^{-1/(\Delta - 1)}$ (or equivalently the
bound on $p$ can be lowered). However, as in the proof of
Theorem~\ref{thm:main-theorem-gnp} we use it in order to embed a graph $H$ with
$\Delta(H) \leq 3$ into $(\eps, p)$-regular subgraphs we cannot allow that to be
the case (see the discussion in Section~\ref{sec:strategy-trees}); in
particular, we are not able to maintain properties
\ref{stable-large-neighbourhoods} and \ref{stable-regularity-inheritance} by
extending $\psi$ into $\phi$. Thus, we resort to a simpler variant of the
statement.

\begin{proof}
  Without loss of generality assume that $\xi > 0$ is as small as necessary; in
  particular, say $0 < \xi < 1/8$. The proof closely follows the first free
  bucket embedding strategy presented in the proof of
  Lemma~\ref{lem:tree-embedding-lemma}. Given $\alpha$ and $\mu$, let $\delta =
  \alpha\mu$, $\gamma = (1/6 - \delta/2) \mu(\alpha/2)$, $\beta =
  \delta\gamma/4$, $c_0 = \beta$, $c_1 = 2c_0/\gamma = \delta/2$, $c_2 =
  2c_1/\gamma$, and $C = \max{\{C_{\ref{lem:gnp-properties}}(\delta),
  C_{\ref{lem:common-neighbours-expansion}}(\delta)\}}$. Write $\tilde n := \mu
  n$ for convenience. Suppose that $\Gnp$ is such that the conclusions of
  Lemma~\ref{lem:gnp-properties} and Lemma~\ref{lem:common-neighbours-expansion}
  hold with $\delta$ (as $\eps$); this happens with high probability.

  For every $i \in [10]$, let $V_i = V_i^0 \cup V_i^1 \cup V_i^2$ be an
  equipartition of $V_i$ chosen uniformly at random. Since $np \gg \log n$, by
  Chernoff's inequality and a union bound over all $v \in V(G)$ and all $j \in
  \{0, 1, 2\}$, if a vertex $v \in V(G)$ satisfies $|\CS_G^\psi(v) \cap
  V_{c(v)}| \geq \tilde n(\alpha p/2)^{d_v}$ then
  \begin{equation}\label{eq:cs-min-deg}
    |\CS_G^\psi(v) \cap V_{c(v)}^{j}| \geq (1/3 - \delta)\tilde n(\alpha
    p/2)^{d_v},
  \end{equation}
  for all $j \in \{0, 1, 2\}$, where $d_v \in \{0, 1\}$. Let $B_i$ denote the
  set of vertices $S_i \setminus S_{i - 1}$ for every $i \in [t]$. For every
  $B_i$ do the following:
  \begin{enumerate}[label=(\subscript{E}{{\arabic*}}), leftmargin=3em]
    \item\label{H-embedding-step} for every $v \in B_i$ sequentially choose the
      smallest $j \in \{0, 1, 2\}$ for which
      \[
        \big| \CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}^j \big| \geq
        \big| \CS_G^\psi(v) \cap V_{c(v)}^j \big|/2
      \]
    and set $W_v := \CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}^j$, or
    \item\label{H-terminate} if no such set exists, terminate the procedure.
  \end{enumerate}
  In case step~\ref{H-embedding-step} is performed for every $B_i$ and $v \in
  B_i$ we indeed find a copy of $H$ in $G$. In order to see this, observe that
  since $\psi \colon S_{i - 1} \to V(G)$ is an $(\beps, \alpha p, c)$-stable
  embedding at the point of embedding some $v \in B_i$, by
  \ref{stable-large-neighbourhoods} we have $|\CS_G^\psi(v) \cap V_{c(v)}| \geq
  \tilde n(\alpha p/2)^{d_v}$, where $d_v = \deg_H(v, S_{i - 1})$. Therefore, by
  \eqref{eq:cs-min-deg},
  % as
  % $np \gg \log n$, by Chernoff's inequality and a union bound $|\CS_G^\psi(v)
  % \cap V_{c(v)}^j| \geq (1/3 - \delta)\tilde n(\alpha p/2)^{d_v}$ for all $j \in
  % \{0, 1, 2\}$.
  % Consequently,
  the choice of the set $W_v$ as in \ref{H-embedding-step} is such that $|W_v|
  \geq \xi\tilde n(\alpha p/2)^{d_v}$, and there exists a stable embedding $\phi
  \colon S_i \to V(G)$.

  Suppose towards contradiction there is an $i \in [t]$ such that for some $v
  \in B_i$ the process enters \ref{H-terminate}, or equivalently
  \begin{equation}\label{eq:no-candidate-available}
    \big|\CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}^j\big| < \big|\CS_G^\psi(v) \cap
    V_{c(v)}^j\big|/2 \qquad \text{for all $j \in \{0, 1, 2\}$}.
  \end{equation}
  Let $X_j := V_{c(v)}^j \cap \psi(S_{i - 1})$ for all $j \in \{0, 1, 2\}$. In
  other words, $X_j$ is just the set of vertices in $V_{c(v)}^j$ `taken' by the
  embedding of $H[S_{i - 1}]$. Assume that
  \begin{equation}\label{eq:double-star}
    |X_j| \leq
    \begin{cases}
      \beta n, & \text{ if $j = 0$}, \\
      \frac{c_j}{n^{j - 1} p^j}, & \text{ otherwise}.
    \end{cases}
    \tag{$\star\star$}
  \end{equation}
  Observe that for $j = 2$ we have $np^2 > c_2$ which implies $X_2 =
  \varnothing$ and thus $\CS_G^\psi(v, S_{i - 1}) \cap V_{c(v)}^2 =
  \CS_G^\psi(v) \cap V_{c(v)}^2$---a contradiction with
  \eqref{eq:no-candidate-available}. Hence, it remains to prove
  \eqref{eq:double-star}.

  Since $v(H) \leq \beta n$ the claim is trivially true for $j = 0$. Consider
  the smallest $j \in \{1, 2\}$ for which \eqref{eq:double-star} fails. The goal
  is to show that the set $X_{j - 1}$ then violates it as well, which
  contradicts our assumption that $j$ is the smallest such index.

  For every $x \in X_j$ set $v_x = \psi^{-1}(x)$ and $q_x = \psi(N_H(v_x, S_{k -
  1}))$, where $v_x \in B_k$ for some $k < i$. Namely, $q_x$ is the image of
  a vertex (and note there can be at most one by the assumption of the lemma)
  whose embedding `forces' $v_x$ to be embedded into $X_j$. Let $Q = \bigcup_{x
  \in X_j} q_x$. Because every $v_x$ gets embedded into $X_j$ and not $X_{j -
  1}$, for $d_{v_x} = \deg_H(v_x, S_{k - 1})$ we have
  \begin{equation}\label{eq:taken}
    \big|\CS_G^\psi(v_x) \cap V_{c(v_x)}^{j - 1} \cap \psi(S_{k - 1}) \big| \geq
    |\CS_G^\psi(v_x) \cap V_{c(v_x)}^{j - 1}|/2
    \osref{\ref{stable-large-neighbourhoods}, \eqref{eq:cs-min-deg}}\geq (1/6 -
    \delta/2)\tilde n(\alpha p/2)^{d_{v_x}} \geq \gamma np,
  \end{equation}
  for $\gamma$ as defined, where in the last inequality we use the fact
  that $\deg_H(v_x, S_{k - 1}) \leq 1$. Since $\CS_G^\psi(v_x, V_{c(v_x)}^{j -
  1})
  \subseteq N_G(q_x) \subseteq N_\Gamma(q_x)$ for every $x \in X_j$, we have
  \begin{equation}\label{eq:mess-strikes-back}
    |N_G(Q, V_{c(v_x)}^{j - 1})| \geq |N_\Gamma(Q)| - \Big| \bigcup_{x \in X_j}
    N_\Gamma(q_x) \setminus \big( \CS_G^\psi(v_x) \cap V_{c(v_x)}^{j - 1} \cap
    \psi(S_{k - 1}) \big) \Big|.
  \end{equation}
  As $|Q| = |X_j|$, which we can further assume to be of size precisely
  $c_j/(n^{j - 1}p^j) < \delta/p$, we derive $|N_\Gamma(Q)| \geq (1 -
  \delta)|X_j|np$ from Lemma~\ref{lem:common-neighbours-expansion} applied with
  $\delta$ (as $\eps$) and $Q$ (as $\cP$). For the second term making use of
  Lemma~\ref{lem:gnp-properties} with $\delta$ (as $\eps$) and \eqref{eq:taken},
  we get
  \[
    \Big| \bigcup_{x \in X_j} N_\Gamma(q_x) \setminus \big( \CS_G^\psi(v_x) \cap
    V_{c(v_x)}^{j - 1} \cap \psi(S_{k - 1}) \big) \Big| \leq |X_j| \cdot (1 +
    \delta)np - |X_j| \cdot \gamma np.
  \]
  Therefore, we can bound the right-hand side of~\eqref{eq:mess-strikes-back},
  to obtain
  \[
    |X_{j - 1}| \geq |N_G(Q, V_{c(v_x)}^{j - 1})| \geq (1 - \delta)|X_j|np -
    |X_j| \big( (1 + \delta)np - \gamma np \big) \geq
    |X_j| \cdot \gamma np/2.
  \]
  Finally, by using a bound on $|X_j|$ given by \eqref{eq:double-star}, we
  arrive at
  \[
    |X_{j - 1}| > \frac{c_j}{n^{j - 1}p^j} \cdot \frac{\gamma np}{2} =
    \frac{c_{j - 1}}{n^{j - 2} p^{j - 1}},
  \]
  which is the desired contradiction. This completes the proof.
\end{proof}


==> ramsey_universal.tex <==
%!TEX root = size_ramsey.tex
\section{Ramsey universality of random graphs}
\label{sec:main-proof}

In this section we give the proof of Theorem~\ref{thm:main-theorem-gnp}. We
start with an arbitrary $2$-colouring of the edges of $\Gamma$ which naturally
partitions the edge set into graphs $\Gamma_r$ and $\Gamma_b$. As many
favourable properties regarding the distribution of edges (and other structures)
may be completely void when considering only, say, $\Gamma_r$, we restore some
of them by utilising the sparse regularity lemma
(Theorem~\ref{thm:sparse-regularity-lemma}). Such an approach has first been
used by Chv\'{a}tal, R\"{o}dl, Szemer\'{e}di, and
Trotter~\cite{chvatal1983ramsey}.

The rest of the general strategy follows the same steps as in previous works
such as~\cite{conlon1size, kohayakawa2011sparse}. After applying the sparse
regularity lemma (Theorem~\ref{thm:sparse-regularity-lemma}) to, say, $\Gamma_r$
we obtain an $(\eps, p)$-regular partition $(V_i)_{i = 0}^{t}$ of $V(\Gamma_r)$.
Additionally, due to sharp concentration of the edges between linear-sized sets
in $\Gnp$, such a partition is $(2\eps, p)$-regular in $\Gamma_b$ as well.
Consider the reduced graph $F$ on vertex set $[t]$ with edges $ij \in F$ if
$(V_i, V_j)$ is an $(2\eps, p)$-regular pair in $\Gamma_b$ (thus also
$\Gamma_r$). Tur\'{a}n's theorem then easily yields a copy of a large complete
graph $K_R$ in $F$, which by colouring each edge $ij \in K_R$ in the majority
colour, say red, from $(V_i, V_j)$, also contains a {\em red copy} of $K_{11}$.
The following lemma consequently shows that such a configuration is highly
likely to be $\cH_3(\beta n)$-universal, completing the proof.

\begin{lemma}\label{lem:main-embedding-lemma}
  For all $\alpha, \mu > 0$ there exist positive constants $\eps(\alpha)$,
  $\beta(\alpha, \mu)$, and $C(\alpha, \mu)$, such that w.h.p.\ a random graph
  $\Gamma \sim \Gnp$ satisfies the following, provided that $p \geq Cn^{-2/5}$.
  Let $G \subseteq \Gamma$ belong to the class $\cG(K_{11}, \tilde n, \eps,
  \alpha p)$, where $\tilde n \geq \mu n$. Then $G$ is $\cH_3(\beta
  n)$-universal.
\end{lemma}

\begin{proof}[Proof of Theorem~\ref{thm:main-theorem-gnp}]
  Let $R = r(K_{11})$ be the smallest integer such that every red-blue colouring
  of the edges of $K_R$ yields a monochromatic copy of $K_{11}$. Let $\alpha =
  1/3$, $\eps' = \eps_{\ref{lem:main-embedding-lemma}}(\alpha)$, $\eps = \min{\{
  1/(3R - 3), \eps'\alpha/2\}}$, $t =
  t_{\ref{thm:sparse-regularity-lemma}}(\eps, R)$, $\mu = (1 - \eps)/t$, and
  $\beta = \beta_{\ref{lem:main-embedding-lemma}}(\alpha, \mu)$. Furthermore,
  choose $C > 0$ large enough so that w.h.p.\ the graph $\Gamma = (V, E)$
  satisfies:
  \begin{itemize}
    \item the conclusion of Lemma~\ref{lem:gnp-properties} with $\eps \cdot \mu$
      (as $\eps$) and $C$, and
    \item the conclusion of Lemma~\ref{lem:main-embedding-lemma} with $\alpha$,
      $\mu$, $\eps'$ (as $\eps$), $\beta$, and $C$.
  \end{itemize}

  Let $E = E_r \cup E_b$ be an arbitrary red-blue colouring of the edges of
  $\Gamma$ and let $\Gamma_i = (V, E_i)$ for $i \in \{r, b\}$. We apply
  Theorem~\ref{thm:sparse-regularity-lemma} to $\Gamma_r$ in order to obtain an
  $(\eps, p)$-regular partition $(V_i)_{i = 0}^{t}$. Let $\tilde n := |V_i|$ and
  note that, since $|V_0| \leq \eps n$, we have $\tilde n \geq (1 - \eps)n/t =
  \mu n$. Additionally, the number of pairs $(V_i, V_j)$ which are $(\eps,
  p)$-regular in $\Gamma_r$ is at least
  \begin{equation}\label{eq:num-edges-regular-pairs}
    \binom{t}{2} - \eps t^2 \geq \frac{t (t - 1)}{2} - \eps t^2 \geq \frac{(1 -
    3\eps)t^2}{2} \geq \Big( 1 - \frac{1}{R - 1} \Big)\frac{t^2}{2}.
  \end{equation}
  Note that, by the properties of regular pairs and as $e_\Gamma(V_i, V_j) = (1
  \pm \eps \mu) \tilde n^2 p$, every pair $(V_i, V_j)$ which is $(\eps,
  p)$-regular in $\Gamma_r$ is $(2\eps, p)$-regular in $\Gamma_b$.

  Consider a graph $F$ on the vertex set $[t]$ where $ij \in F$ if $(V_i, V_j)$
  is $(2\eps, p)$-regular in $\Gamma$, and additionally is coloured red if
  $e_{\Gamma_r}(V_i, V_j) \geq e_{\Gamma_b}(V_i, V_j)$, and blue otherwise.
  By~\eqref{eq:num-edges-regular-pairs} we have that $e(F) \geq \big(1 - 1/(R -
  1)\big) v(F)^2 / 2$ and thus by Tur\'{a}n's theorem, $F$ contains $K_R$ as a
  subgraph. Moreover, by Ramsey's theorem, $K_R$ (and thus $F$) contains a {\em
  monochromatic} copy of $K_{11}$ in colour $c \in \{r, b\}$. By relabelling if
  necessary, we may assume that the $K_{11}$ is given by the vertices $\{1,
  \dotsc, 11\}$. In particular, for all $1 \leq i < j \leq 11$ we have
  \begin{itemize}
    \item $(V_i, V_j)$ is $(2\eps, p)$-regular in $\Gamma_c$, and
    \item $e_{\Gamma_c}(V_i, V_j) \geq e_\Gamma(V_i, V_j)/2 \geq (1 -
      \eps\mu)\tilde n^2 p/2 \geq \alpha \tilde n^2 p$.
  \end{itemize}

  As every $(2\eps, p)$-regular pair with density at least $\alpha p$ is
  $(2\eps/\alpha, \alpha p)$-lower-regular, we deduce that $\Gamma_c[V_1 \cup
  \dotsb \cup V_{11}]$ belongs to the class $\cG(K_{11}, \tilde n, \eps', \alpha
  p)$. Finally, by Lemma~\ref{lem:main-embedding-lemma} the graph $\Gamma_c[V_1
  \cup \dotsb \cup V_{11}]$ is $\cH_3(\beta n)$-universal, which completes the
  proof.
\end{proof}

In the remainder of the section we provide a highly technical proof of
Lemma~\ref{lem:main-embedding-lemma}.

\begin{proof}[Proof of Lemma~\ref{lem:main-embedding-lemma}]
  Given $\alpha$ and $\mu$ we define numerous constants that are used in the
  proof. Let $\xi = 1/17$, $\eps^\star = \eps_6 = \min{\{\frac{1}{28},
  \eps_{\ref{thm:klr-random-graphs}}(K_4)\}}$ and for all $i = 5, \dotsc, 0$ let
  \[
    \eps_i = \frac{\xi}{2} \cdot \min \big\{ \eps_{i + 1},
      \eps'_{{\ref{prop:one-sided-inheritance}}}(\tfrac{\alpha}{2}),
      %
      \eps^\star_{{\ref{prop:one-sided-inheritance}}}(\tfrac{\alpha}{2}),
      %
      \eps^\star_{\ref{prop:two-sided-inheritance}}(\alpha, \eps_{i + 1}),
      %
      \eps'_{\ref{prop:double-inheritance}}(\alpha),
      %
      \eps^\star_{\ref{prop:double-inheritance}}(\alpha, \eps_{i + 1}),
      %
      \eps_{\ref{lem:cycle-embedding-lemma}}(\tfrac{\alpha}{2}) \big\},
  \]
  in particular $0 < \eps_0 < \eps_1 < \dotsb < \eps_5 < \eps^\star < 1$, and
  let $\eps = \eps_0$. As $\Delta(H) \leq 3$, this defines a $6$-tuple $\beps =
  (\eps_0, \eps_1, \dotsc, \eps_5)$. Let $\beta = \min{\{
    \beta_{\ref{lem:tree-embedding-lemma}}(\tfrac{\alpha}{2},
    \tfrac{\xi\mu\alpha}{4}),
    \beta_{\ref{lem:cycle-embedding-lemma}}(\tfrac{\alpha}{2},
    \tfrac{\xi\mu\alpha}{4}),
    \beta_{\ref{lem:magic-embedding-lemma}}(\alpha, \mu),
    \tfrac{\eps_0}{2}
  \}}$.

  Since $\Delta(H) \leq 3$ there may exist {\em isolated copies of $K_4$} in
  $H$. Recall, $m_2(K_4) = 5/2$ and as w.h.p.\ $G$ satisfies the conclusion of
  Proposition~\ref{thm:klr-random-graphs} for $K_4$ (as $H$) and $\tilde n$ (as
  $n$), we can (greedily) embed $\beta n$ vertex-disjoint copies of $K_4$ into
  $G$. As $\beta \ll \eps^\star$ by removing all the vertices used for the
  embedding, the `regularity' between classes of $G$ essentially does not
  change. Therefore, we assume throughout that $H$ is $K_4$-free.

  \paragraph*{Preparing $H$.} We aim to make use of
  Lemma~\ref{lem:magic-embedding-lemma} to find an embedding of $H$ into $G$. In
  order to do that, we first have to find a chain $\varnothing = S_0 \subset S_1
  \subset \dotsb \subset S_t = V(H)$, for some $t > 0$, such that
  \begin{equation}\label{eq:deg-requirement-H}
    \deg_H(v, S_{i - 1}) \leq 1, \qquad \text{for all $i \in [t]$ and $v \in S_i
    \setminus S_{i - 1}$}.
  \end{equation}
  However, an arbitrary such chain does not work out of the box, as we need to
  further ensure we can embed each $H[S_i \setminus S_{i - 1}]$ into $G$ in a
  prescribed way, that is so that every stable embedding of $H[S_{i - 1}]$ can
  be extended to a stable embedding of $H[S_i]$. For that the graphs $H[S_i
  \setminus S_{i - 1}]$ need to have a suitable structure.

  Let $\{X_i\}_{i \in [x]}$, for some $x \leq \beta n$, be a maximal
  disjoint family of subsets of $V(H)$, in which each $X_i$ induces a cycle of
  length at least four in $H$. Let $T = H \setminus H[\bigcup_{i \in [x]} X_i
  ]$ denote the graph that remains and without loss of generality assume that
  $T$ is connected. Then, $T$ is a `triangle-tree'---a tree where every vertex
  is blown-up into either a triangle or a $K_4 \setminus e$, preserving
  $\Delta(T) \leq 3$. \MT{Should I prove this or this is obvious enough?}

  Let $r \in V(T)$ be a vertex for which $N_H(r)$ does not induce a path of
  length two in $H$. Such a vertex always exists as $T$ is $K_4$-free and
  $\Delta(T) \leq 3$. Root $T$ at $r$ and consider the `BFS-tree' that naturally
  arises. For every $v \in T$ we let $\mathrm{dist}(v, r)$ denote the length (in
  the number of edges) of the shortest path between $v$ and $r$ in $T$. For
  every copy of $K_4 \setminus e$ in $T$ mark one of the degree-three vertices
  in $K_4 \setminus e$ and let $Y_1$ consist of all such marked vertices. Note
  that $H[Y_1]$ is an independent set. Next, for every triangle on vertices
  $v_1, v_2, v_3$ which does not belong to a copy of $K_4 \setminus e$ and where
  $\mathrm{dist}(r, v_1) < \mathrm{dist}(r, v_2) = \mathrm{dist}(r, v_3)$, `cut'
  the vertex $v_1$ from the edge $v_2v_3$ by artificially removing the edges
  $v_1v_2$ and $v_1v_3$. This partitions $V(T) \setminus Y_1$ into sets $Y_2,
  \dotsc, Y_y$, for some $y \leq \beta n$. By relabelling if necessary,
  assume that the order of $Y_i$'s is chosen such that for every $2 \leq i < j
  \leq y$
  \[
    \min_{v \in Y_i} \mathrm{dist}(v, r) \leq \min_{u \in Y_j} \mathrm{dist}(u,
    r),
  \]
  where ties are broken arbitrarily. This produces a partition of $V(T)$ for
  which:
  \begin{enumerate}[label=(H\arabic*), font=\itshape, leftmargin=3em]
    \item\label{h-tree} $T[Y_i]$ is a tree, for all $i \geq 1$,
    \item\label{h-back-deg} $\deg_H(v, \bigcup_{j < i} Y_j) \leq 1$ for every $i
      \in [y]$ and $v \in Y_i$, and
    \item\label{h-edge} $\deg_H(v, \bigcup_{j < i} Y_j) = 0$ for every $i \in
      [y]$ and $v \in Y_i$ for which $e_H(N_H(v) \setminus \bigcup_{j < i} Y_j))
      > 0$.
  \end{enumerate}
  Perhaps the least obvious one being \ref{h-edge}, which is trivially satisfied
  for all $v \in Y_1$. Note that a vertex $v \in Y_i$ which violates
  \ref{h-edge} and an edge $uw \in N_H(v) \setminus \bigcup_{j < i} Y_i$,
  necessarily need to belong to different $Y_i$'s by construction. As
  $\delta(T[Y_i]) \geq 1$ for all $i \geq 2$, existence of such a vertex $v$
  would then also violate the degree constraint $\Delta(H) \leq 3$.

  An example of a partition of $V(T)$ as given by the procedure described above
  is depicted in Figure~\ref{fig:H-partition}.

  \begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.8]{figures/H-partition}
    \caption{An example of a graph $H$ with a partition of its triangle-tree
    into $Y_1, \dotsc, Y_6$ in grey (on the left). The red vertices are the
    marked ones and go into $Y_1$ and the red lines show how to cut the
    triangles. An induced cycle of length eight and a possible way of it being
    connected to the triangle-tree (on the right).}
    \label{fig:H-partition}
  \end{figure}

  Setting $S_i = \bigcup_{j = 1}^{i} Y_i$ for all $i \in [y]$ and $S_{y + i}
  = S_y \cup \bigcup_{j = 1}^{i} X_i$ for all $i \in [x]$ finishes the
  construction of a chain which satisfies \eqref{eq:deg-requirement-H} as
  desired and which is particularly suitable for the embedding as we show next.

  \paragraph*{Embedding $H$ into $G$.} Let $c \colon V(H^2) \to [10]$ be a
  proper colouring of the graph $H^2$---a graph obtained from $H$ by adding an
  edge between every pair of vertices at distance two in $H$. We embed $H$ into
  $G$ such that every vertex $v \in V(H)$ gets mapped to a vertex belonging to
  $V_{c(v)}$. The set $V_{11}$ is there just for technical reasons and in order
  to make the exposition cleaner---we use some of its vertices as $\{s_1,
  \dotsc, s_t\}$ in Lemma~\ref{lem:tree-embedding-lemma} and
  Lemma~\ref{lem:cycle-embedding-lemma} to embed trees and cycles.

  Throughout, we assume that $\Gnp$ is such that
  \begin{enumerate}[label=(R\arabic*), font=\itshape, leftmargin=3em]
    \item\label{R-one-sided-inheritance} the conclusion of
      Proposition~\ref{prop:one-sided-inheritance} holds for $G$ with $\eps_{i +
      1}$ (as $\eps$), $\alpha/2$ (as $\alpha$), $\xi\mu/2$ (as $\mu$), and
      $2\eps_j/\xi$ (as $\eps'$) and $2\eps_i/\xi$ (as $\eps^\star$), for all
      $i, j \in [5]$;
    \item\label{R-two-sided-inheritance} the conclusion of
      Proposition~\ref{prop:two-sided-inheritance} holds for $G$ with $\eps_{i +
      1}$ (as $\eps$), $\alpha$, $\xi\mu$ (as $\mu$), and $\eps_i/\xi$ (as
      $\eps^\star$), for all $i \in [5]$;
    \item\label{R-double-inheritance} the conclusion of
      Proposition~\ref{prop:double-inheritance} holds for $G$ with $\eps_{i +
      j}$ (as $\eps$), $\alpha$, $\xi\mu\alpha/2$ (as $\mu$), $\max{\{\eps_i,
      \eps_j\}}$ (as $\eps'$), and $\eps_0$ (as $\eps^\star$), for all $i, j \in
      \{0, 1\}$;
    \item\label{R-trees} the conclusion of Lemma~\ref{lem:tree-embedding-lemma}
      holds for $G$ with $\alpha/2$ (as $\alpha$), $\xi\mu\alpha/4$ (as $\xi$),
      and $\beta$;
    \item\label{R-cycles} the conclusion of Lemma~\ref{lem:cycle-embedding-lemma}
      holds for $G$ with $\alpha/2$ (as $\alpha$), $\xi\mu\alpha/4$ (as $\xi$),
      $\beta$, and $\eps_2$ (as $\eps$).
  \end{enumerate}
  By our choice of constants and for a large enough $C > 0$, as $p \geq
  Cn^{-2/5}$, \ref{R-one-sided-inheritance}--\ref{R-cycles} hold simultaneously
  with high probability.

  The rest of the embedding proceeds by inductively showing that the assumptions
  of the Embedding Lemma (Lemma~\ref{lem:magic-embedding-lemma}) hold. We aim to
  show the following for every $i \in [t]$: given an arbitrary $(\beps, \alpha
  p, c)$-stable embedding $\psi \colon S_{i - 1} \to V(G)$ and, for every $v \in
  S_i \setminus S_{i - 1}$, subsets $W_v \subseteq \CS_G^\psi(v, S_{i - 1}) \cap
  V_{c(v)}$ of size $|W_v| \geq \xi\tilde n (\alpha p/2)^{\deg_H(v, S_{i -
  1})}$, we can extend it to an $(\beps, \alpha p, c)$-stable embedding $\phi
  \colon S_i \to V(G)$ which maps every $v \in S_i \setminus S_{i - 1}$ into
  some $\phi(v) \in W_v$.

  As every embedding of $S_0$ is trivially $(\beps, \alpha p, c)$-stable, we
  assume that we can do it for all $S_0 \subset \dotsb \subset S_{i - 1}$ and
  let us show it for $i \geq 1$. Let $W_v \subseteq \CS_G^\psi(v, S_{i - 1})
  \cap V_{c(v)}$ be subsets of size $|W_v| = \xi \tilde n(\alpha p/2)^{\deg_H(v,
  S_{i - 1})}$.

  For convenience, in the remainder we write $B_i := S_i \setminus S_{i - 1}$.
  The following claim is slightly technical and follows from several usages of
  regularity inheritance properties
  \ref{R-one-sided-inheritance}--\ref{R-double-inheritance}, so we postpone its
  proof for the sake of a cleaner exposition.

  \begin{claim}\label{cl:good-vertices}
    There exists a collection $\{Q_v\}_{v \in B_i}$ of (not necessarily
    disjoint) sets $Q_v \subseteq W_v$ of size $|Q_v| = |W_v|/2$ such that
    setting $\phi(v) = x$ for any $x \in Q_v$
     satisfies:
    \begin{enumerate}[(i)]
      \item\label{cl-vertex} $|\CS_G^\phi(u) \cap V_{c(u)}| \geq \tilde n
        (\alpha p/2)^{d_u}$, for every $u \in V(H) \setminus S_i$, where
        $d_u = \deg_H(u, S_i)$, and
      \item\label{cl-edge} $\big( \CS_G^\phi(u) \cap V_{c(u)}, \CS_G^\phi(w)
        \cap V_{c(w)} \big)$ is $(\eps_{d_{uw}}, \alpha p)$-lower-regular for
        every $uw \in H[V(H) \setminus S_i]$, where $d_{uw} = \deg_H(u, S_i) +
        \deg_H(w, S_i)$.
    \end{enumerate}
  \end{claim}

  In other words, the claim above allows us to maintain both
  \ref{stable-large-neighbourhoods} and \ref{stable-regularity-inheritance} by
  embedding every $v \in B_i$ into its corresponding set $Q_v$. Moreover, as
  property \ref{stable-colour-class} is given for free by the fact that $Q_v
  \subseteq W_v \subseteq \CS_G^\psi(v) \cap V_{c(v)}$, the only thing that
  remains to be taken care of is to find suitable images for the vertices of
  $B_i$ in $\bigcup_{v \in B_i} Q_v$ which preserve
  \ref{stable-embedding-edges}. In order to do this, we need to consider two
  cases: $H[B_i]$ is a tree (see~\ref{h-tree}) or $H[B_i]$ is a cycle of length
  at least four.
  % As the first is trivial we focus on the latter two.

  The preparation for the embedding is essentially the same for both cases, in
  the end it only boils down to which of the two properties \ref{R-trees} or
  \ref{R-cycles} do we apply. Assume $B_i = \{v_1, \dotsc, v_\ell\}$, for some
  $\ell \geq 1$, is a $1$-degenerate ordering of the vertices of $H[B_i]$ if it
  is a tree and otherwise just an orientation of a cycle (in which case $\ell
  \geq 4$). Recall, for every $v_j \in B_i$, $\deg_H(v_j, S_{i - 1}) \leq 1$.
  Let $s_j$ be the image under $\psi$ of this unique neighbour if it exists and
  let $J \subseteq [\ell]$ be the indices of the vertices in $B_i$ which have no
  neighbour in $S_{i - 1}$. Greedily, for every $j \in J$, take $s_j$ to be a
  vertex (disjoint from all other $s_j$'s) belonging to $V_{11}$ such that
  \begin{itemize}
    \item $|N_G(s_j, V_{c(v_j)})| \geq \tilde n (\alpha p/2)$, and
    \item $\big( N_G(s_j, V_{c(v_j)}), Q_{v_z} \big)$ is $(\eps_2, \alpha
      p)$-lower-regular for all $v_jv_z \in H[B_i]$ with $z \in [\ell] \setminus
      J$, and
    \item $\big( N_G(s_j, V_{c(v_j)}), N_G(s_q, V_{c(v_q)}) \big)$ is $(\eps_2,
      \alpha p)$-lower-regular for all $v_jv_q \in H[B_i]$ with $q \in J$.
  \end{itemize}
  In order to see that such a choice of vertices exists, consider some $v_z \in
  B_i$ for $z \in [\ell] \setminus J$ and $v_jv_z \in B[H_i]$---the proof for
  $v_q$ with $q \in J$ is analogous. Due to $\Delta(H) \leq 3$, at most three
  such vertices $v_z$ exist. Since $\psi$ is a stable embedding, from
  \ref{stable-large-neighbourhoods}, \ref{stable-regularity-inheritance}, and
  Proposition~\ref{prop:large-subset-reg-inheritance} it follows that
  $(V_{c(v_j)}, Q_{v_z})$ is $(2\eps_1/\xi, \alpha p)$-lower-regular. Thus, by
  property \ref{R-one-sided-inheritance} there are at least $(1 -
  3\eps_2)|V_{11}|$ vertices $s_j \in V_{11}$ so that $|N_G(s_j, V_{c(v_j)})|
  \geq \tilde n(\alpha p/2)$ and all $\big( N_G(s_j, V_{c(v_j)}), Q_{v_z} \big)$
  and $\big( N_G(s_j, V_{c(v_j)}), N_G(s_q, V_{c(v_q)}) \big)$ are $(\eps_2,
  \alpha p)$-lower-regular simultaneously for $v_z$ and $v_q$ as desired. As
  $\ell \leq \beta n$, and $|V_{11}| \geq \mu n$, there is always a choice for
  such a vertex $s_j$. Recall, for every $z \in [\ell] \setminus J$, $|Q_{v_z}|
  = (\xi/2)\tilde n(\alpha p/2)$. Consequently, for every $q \in J$ let $U_q$ be
  a subset of $N_G(s_q, V_{c(v_q)})$ of size precisely $(\xi/2)\tilde n(\alpha
  p/2)$, and for every $z \in [\ell] \setminus J$ let $U_z = Q_{v_z}$. This is
  sufficient to apply \ref{R-cycles} if $H[B_i]$ is a cycle, with $\{s_1,
  \dotsc, s_\ell\}$ and $U_1, \dotsc, U_\ell$ (as $V_1, \dotsc, V_\ell$) to find
  a canonical copy of $H[B_i]$ in $G[Q_{v_1} \cup \dotsb \cup Q_{v_\ell}]$ as
  required.

  On the other hand, if $H[B_i]$ is a tree, we need to ensure that for every
  $v_j$ and its unique neighbour $v_{a(j)}$ in the degenerate ordering with
  $a(j) < j$, the pair $(U_{a(j)}, U_j)$ is such that all $u \in U_{a(j)}$
  satisfy $\deg_G(u, U_j) \geq (1 - \eps^\star)|U_j|\alpha p$ (see
  Lemma~\ref{lem:tree-embedding-lemma}~$\ref{emb-tree-degree}$). For every $v_j$
  with $\deg_{H[B_i]}(v_j, \{v_{j + 1}, \dotsc, v_\ell\}) = 0$, let $U_j'
  \subseteq U_j$ be of size $|U_j'| = |U_j|/2$. As every $(U_{a(j)}, U_j)$ is,
  with room to spare, $(2\eps_2/\xi, \alpha p)$-lower-regular, there is a set
  $U_{a(j)}' \subseteq U_{a(j)}$ of size $|U_{a(j)}|/2$ (with room to spare)
  consisting only of vertices $u$ satisfying $\deg_G(u, U_j') \geq (1 -
  \eps^\star)|U_j'|\alpha p$. This `cleaning' can be done by starting from
  $U_\ell$ and going to $U_1$ without harming the regularity between sets
  significantly---every such pair $(U_{a(j)}', U_j')$ becomes $(\eps^\star,
  \alpha p)$-lower-regular (with room to spare again). Subsequently, we apply
  property \ref{R-trees} to find a canonical copy of $H[B_i]$ in $G[U_1' \cup
  \dotsb \cup U_\ell']$.

  It remains to prove Claim~\ref{cl:good-vertices}.

  \begin{proof}[Proof of Claim~\ref{cl:good-vertices}]
    Consider $v \in B_i$, let $d_v = \deg_H(v, S_{i - 1})$, and note that $d_v
    \in \{0, 1\}$. For every $u \in N_H(v) \setminus S_i$, it holds that
    $\deg_H(u, S_{i - 1}) = 0$. Since $\psi$ is an $(\beps, \alpha p, c)$-stable
    embedding of $H[S_{i - 1}]$, by property~\ref{stable-regularity-inheritance}
    and Proposition~\ref{prop:large-subset-reg-inheritance}, $(W_v,
    \CS_G^\psi(u) \cap V_{c(u)})$ is $(\eps_{d_v}/\xi, \alpha p)$-lower-regular.
    Moreover, $|\CS_G^\psi(u) \cap V_{c(u)}| = |V_{c(u)}| = \tilde n$.
    Therefore, as $\Delta(H) \leq 3$, there are at least $(1 -
    3\eps_{d_v}/\xi)|W_v|$ vertices $x \in W_v$ for which setting $\phi(v) := x$
    satisfies
    \[
      |\CS_G^\phi(u) \cap V_{c(u)}| = |N_G(x, V_{c(u)})| \geq (1 -
      \eps_{d_v}/\xi)|V_{c(u)}|\alpha p \geq \tilde n (\alpha p/2),
    \]
    for all $u \in N_H(v) \setminus S_i$ simultaneously, establishing
    $\ref{cl-vertex}$.

    Consider now an edge $uw \in H[V(H) \setminus S_i]$. If $N_H(u, B_i) \cup
    N_H(w, B_i) = \varnothing$ then embedding $H[B_i]$ does not affect the
    candidate sets $\CS_G^\phi(u)$ and $\CS_G^\phi(w)$ nor the regularity
    between them. Assume first $uw \in H[N_H(v)]$. Crucially, by \ref{h-edge},
    $d_v = 0$ and $\deg_H(u, S_{i - 1}) = \deg_H(w, S_{i - 1}) = 0$. This in
    particular implies that, by \ref{stable-large-neighbourhoods} and
    \ref{stable-regularity-inheritance},
    \[
      |W_v| = \xi\tilde n, \qquad |\CS_G^\psi(u) \cap V_{c(u)}| = \tilde n,
      \qquad \text{and} \qquad |\CS_G^\psi(w) \cap V_{c(w)}| = \tilde n,
    \]
    and
    \[
      (W_v, \CS_G^\psi(u) \cap V_{c(u)}), \quad (W_v, \CS_G^\psi(w) \cap
      V_{c(w)}), \quad \text{and} \quad (\CS_G^\psi(u) \cap V_{c(u)},
      \CS_G^\psi(w) \cap V_{c(w)})
    \]
    are all $(\eps_0/\xi, \alpha p)$-lower-regular. Hence, by
    \ref{R-two-sided-inheritance}, there are at least $(1 - \eps_1)|W_v|$
    vertices $x \in W_v$ for which setting $\phi(v) := x$ satisfies that $\big(
    \CS_G^\phi(u) \cap V_{c(u)}, \CS_G^\phi(v) \cap V_{c(w)} \big)$ is $(\eps_1,
    \alpha p)$-lower-regular, which is sufficient for $\ref{cl-edge}$ as
    $\deg_H(u, S_i) + \deg_H(w, S_i) = 2$ and $\eps_1 < \eps_2$.

    Next, if $uw$ is such that $\deg_H(u, B_i) = 1$ and $\deg_H(w, B_i) = 0$, we
    do as follows. Let $d_w = \deg_H(w, S_{i - 1})$. As $\psi$ is an $(\beps,
    \alpha p, c)$-stable embedding of $H[S_{i - 1}]$, we have
    \[
      |W_v| = \xi\tilde n(\alpha p/2)^{d_v}, \qquad |\CS_G^\psi(u) \cap
      V_{c(u)}| = \tilde n, \qquad \text{and} \qquad |\CS_G^\psi(w) \cap
      V_{c(w)}| \geq \tilde n(\alpha p/2)^{d_w}.
    \]
    Moreover, $(W_v, \CS_G^\psi(u) \cap V_{c(u)})$ is $(\eps_{d_v}/\xi, \alpha
    p)$-lower-regular and $(\CS_G^\psi(u) \cap V_{c(u)}, \CS_G^\psi(w) \cap
    V_{c(w)})$ is $(\eps_{d_w}, \alpha p)$-lower-regular. Hence, as $\Delta(H)
    \leq 3$ and all of $c(v)$, $c(u)$, and $c(w)$ are distinct, property
    \ref{R-one-sided-inheritance} shows that there are at least $(1 -
    6\eps^\star)|W_v|$ vertices $x \in W_v$ for which setting $\phi(v) := x$
    satisfies that $(\CS_G^\phi(u) \cap V_{c(u)}, \CS_G^\phi(w) \cap V_{c(w)})$
    is $(\eps_{d_w + 1}, \alpha p)$-lower-regular, as promised by
    $\ref{cl-edge}$.

    Lastly, if there are $v', v'' \in B_i$ such that $u \in N_H(v') \setminus
    S_i$ and $w \in N_H(v'') \setminus S_i$ we make use of property
    \ref{R-double-inheritance}. Let
    \[
      d_{v'} = \deg_H(v', S_{i - 1}), \enskip d_{v''} = \deg_H(v'', S_{i - 1}),
      \enskip d_u = \deg_H(u, S_{i - 1}), \enskip \text{and} \enskip d_w =
      \deg_H(w, S_{i - 1}).
    \]
    Note that $d_u = d_w = 0$. Again by the fact that $\psi$ is an $(\beps,
    \alpha p, c)$-stable embedding, we have
    \[
      |W_{v'}| = \xi\tilde n(\alpha p/2)^{d_{v'}}, \qquad |W_{v''}| = \xi\tilde
      n(\alpha p/2)^{d_{v''}}, \qquad |V_{c(u)}| = \tilde n, \qquad \text{and}
      \qquad |V_{c(w)}| = \tilde n.
    \]
    Moreover $(W_{v'}, V_{c(u)})$ is $(\eps_{d_{v'}}/\xi, \alpha
    p)$-lower-regular, $(W_{v''}, V_{c(w)})$ is $(\eps_{d_{v''}}/\xi, \alpha
    p)$-lower-regular, and $(V_{c(u)}, V_{c(w)})$, is $(\eps_0, \alpha
    p)$-lower-regular. Thus, \ref{R-double-inheritance} implies that there are
    at least $(1 - \eps^\star)|W_{v'}|$ vertices $x' \in W_{v'}$ and $(1 -
    \eps^\star)|W_{v''}|$ vertices $x'' \in W_{v''}$ such that setting $\phi(v')
    := x'$ and $\phi(v'') := x''$ satisfies that $(\CS_G^\phi(u) \cap V_{c(u)},
    \CS_G^\phi(w) \cap V_{c(w)})$ is $(\eps_2, \alpha p)$-lower-regular, as
    required by $\ref{cl-edge}$. However, note that there may be more pairs $v',
    v''$ in $B_i$ for which this is the case---for every fixed $v'$, there can
    be at most three such vertices $v''$. Greedily finding sets as above for
    every such pair suffices, in which case we lose an additive factor of
    $2\eps^\star$ in the number of vertices $x', x''$. This plays no significant
    role.

    Combining everything above, we conclude that for every $v \in B_i$ there is
    a set $Q_v \subseteq W_v$ of size at least (with room to spare)
    \[
      |W_v| - (3\eps_{d_{v}}/\xi)|W_v| - \eps_1|W_v| - 6\eps^\star|W_v| -
      3\eps^\star|W_v| \geq (1 - 13\eps^\star)|W_v| \geq |W_v|/2,
    \]
    such that setting $\phi(v) := x$ for an arbitrary $x \in Q_v$ maintains both
    $\ref{cl-vertex}$ and $\ref{cl-edge}$, completing the proof of the claim.
  \end{proof}

  This finally concludes the proof of the induction step and hence by
  Lemma~\ref{lem:magic-embedding-lemma} there exists an embedding of $H$ into
  $G$ as required.
\end{proof}


==> sparse_regularity.tex <==
%!TEX root = size_ramsey.tex
\subsection{Regularity inheritance}
\label{sec:sparse_reg}

\RN{Pogledaj, menjaj, i dodaj dokaz Leme \ref{lem:typical_vertices}.}

When dealing with regular pairs in random graphs, we usually cannot claim that something holds for all vertices, but for almost all. This section summarises statements of this type that are used in the main proof, as well as some other standard fact about regular pairs.

The first propositions is usually referred to as a \emph{slicing lemma} and follows directly from the definition of
an $(\eps)$-regularity.

\begin{proposition}\label{prop:large-subset-reg-inheritance}
  Let $0 < \eps_1 < \eps_2 \leq 1/2$, $p \in (0, 1)$, and let $(X, Y)$ be an
  $(\eps_1)$-regular pair in a graph $G$. Then every choice of subsets
  $X' \subseteq X$ and $Y' \subseteq Y$ of size $|X'| \geq \eps_2|X|$ and $|Y'|
  \geq \eps_2|Y|$ forms an $(\eps_1/\eps_2)$-regular pair.
\end{proposition}

In other words, subsets of a regular pair which are not too small induce, again, a regular pair. This allows us to freely take (small linear) subsets as we please and still have an $(\eps)$-regular pairs with $\eps$ as small as we want. We will implicitly use this in the main proof.

The following result of Gerke, Kohayakawa, R\"{o}dl, and Steger~\cite{gerke2007small} enables us to say something about regularity inheritance for subsets of size $o(n)$, for which Proposition \ref{prop:large-subset-reg-inheritance} renders useless.

\begin{lemma}[Corollary 3.9 in~\cite{gerke2007small}]
  \label{lem:small-regularity-inheritance}
  For all $\eps', \beta \in (0, 1)$, there exist positive constants
  $\eps_0(\eps', \beta)$ and $C(\eps')$ such that, for any $0 < \eps \le \eps_0$, the following holds. Let $(V_1, V_2)$ be an $(\eps)$-regular pair of density $p$
  in some graph $G$, and suppose $q_1, q_2 \geq Cp^{-1}$. Let $B$ be the number of pairs $(Q_1, Q_2)$ with $Q_i \subseteq V_i$ and $|Q_i| = q_i$ ($i = 1,2$) and such that there are $\tilde{Q}_i \subseteq Q_i$ with $|\tilde{Q}_i| \ge (1 - \eps')|Q_i|$ for which we have:
  \begin{enumerate}[(i)]
      \item $(\tilde{Q}_1, \tilde{Q}_2)$ is $(\eps')$-regular;
      \item the density $p'$ of $(\tilde{Q}_1, \tilde{Q}_2)$ satisfies $p' \in (1 \pm \eps')p$.
  \end{enumerate}
  Then
  \[
    B \ge (1 - \beta^{\min{\{q_1, q_2\}}}) \binom{|V_1|}{q_1} \binom{|V_2|}{q_2}.
  \]
\end{lemma}

It is rather annoying that one has to consider subsets of $Q_i$'s, rather than the whole sets, however it was shown in \cite{gerke2007small} that this is necessary for the lemma to hold. The conclusion of the lemma is, nonetheless, very powerful: the fraction of pairs of sets of desired size which do not inherit the regularity is extremely small! This is demonstrated in the following lemma. For brevity, we refer to a pair $(Q_1, Q_2)$ with properties $(i)$ and $(ii)$ as described in the previous lemma, with $p$ being implicitly given by the ambient pair, as \emph{$(\eps')$-almost-regular} \RN{Molim te primeti upotrebu reci 'ambient'. Ozbiljna mata, nema zezancije :).}. Moreover, given a pair $(A, B)$ of sets of vertices in some graph, we say that a vertex $a \in A$ is \emph{$B$-typical} (or just typical if $B$ is clear from the context) if it has at least $|B|p/2$ neighbours in $B$, where $p$ is the density of $(A< B)$.

\MT{Evo nase leme:}
\begin{lemma}[Corollary~3.5 in \cite{vskoric2018local}]
  For all $0 < \beta, \eps', d, p < 1$, there exist positive constants
  $\eps_0(\beta,\eps',d)$ and $D(\eps')$, such that for every $0 < \eps \leq
  \eps_0$, the random graph $\GNp$ w.h.p.\ has the following property. Suppose
  $G = (V_1 \cup V_2, E)$ is an $(\eps,p)$-regular \MT{ovo mozemo podesiti}
  graph of density $dp$ which is a subgraph of $\GNp$. Then for all $q_1, q_2
  \geq Dp^{-1}\log N$, there are at least
  \[
    \big(1-\beta^{\min\{q_1,q_2\}}\big) \binom{|V_1|}{q_1} \binom{|V_2|}{q_2}
  \]
  sets $Q_i \subseteq V_i$ of size $|Q_i| = q_i$, $i \in \{1, 2\}$, which induce
  an $(\eps',p)$-regular graph of density $(1 \pm \eps')dp$.
\end{lemma}

\begin{lemma}
  \label{lem:typical_vertices}
  Bla bla random graf $\Gamma  = \Gnp$ bla bla ... :

  Let $G \subseteq \Gamma$ and let $V_1, V_2, V_3, V_4 \subseteq V(G)$ be disjoint sets, each of size $|V_i| = N = \mu n$, such that each pair $(V_i, V_j)$ is $(\eps)$-regular of density $p' = \Theta(p)$, with respect to $G$. Then there exists $V_i' \subseteq V_i$ ($i=1,2,3,4$), each of size $|V_i'| \ge (1 - \eps)|V_i|$, such that the following holds:
  \begin{enumerate}[(P1)]
      \item for every $V_2$-typical vertex $v \in V_1'$, $(N_G(v, V_2), V_3)$ is  $(\eps)$-almost-regular;
      \item for every $v \in V_1'$ which is both $V_2$- and $V_3$-typical, $(N_G(v, V_2), N_G(v, V_3))$ is $(\eps)$-almost-regular;
      \item for every $V_2$-typical $v \in V_1'$ and $V_3$-typical $w \in V_4'$, $(N_G(v, V_2), N_G(w, V_3))$ is $(\eps)$-almost-regular.
  \end{enumerate}
\end{lemma}

\RN{Zapravo ne moramo ni da koristimo rezultat Schachta, ovo nam je cak i lakse. Na pocetku cemo procistiti graf, i onda samo koristimo tipicne cvorove. U dokazu reci da cemo samo pokazati P3, na primer, i dati pun dokaz toga. Precizan dokaz, bez previse zurbe. :-)}

% The power of the lemma above is that it allows for interesting statements about
% certain subsets of vertices in a random graph, as the number of `bad' sets is
% small so that they with high probability do not cause an obstruction. To put
% things into context, suppose $(V_1, V_2)$ and $(V_2, V_3)$ are $(\eps, \alpha
% p)$-lower-regular in a random graph $\Gnp$, for some $\alpha > 0$. Then, most of
% the vertices inside the set $V_1$ are such that their neighbourhood into $V_2$
% is of the `expected size' and is additionally lower-regular with the set $V_3$
% with slightly weaker parameters. This is what in the literature is often
% referred to as the `one-sided inheritance'. A statement similar to the one here
% has been presented and proved in~\cite{kohayakawa2011sparse}.

% \begin{proposition}[Proposition~15 in~\cite{kohayakawa2011sparse}]
%   \label{prop:one-sided-inheritance}
%   For all $\alpha, \eps, \mu > 0$, there exist positive constants
%   $\eps'(\alpha)$\footnote{It is convenient for the proof of
%   Lemma~\ref{lem:main-embedding-lemma} that $\eps'$ does not depend on $\eps$.},
%   $\eps^\star(\alpha, \eps)$, and $C(\alpha, \eps, \mu)$ such that w.h.p.\ a
%   random graph $\Gamma \sim \Gnp$ satisfies the following, provided that $p \geq
%   Cn^{-2/5}$. Let $G \subseteq \Gamma$ and $V_1, V_2, V_3 \subseteq V(G)$ be
%   disjoint sets such that
%   \begin{itemize}
%     \item $(V_1, V_2)$ is $(\eps', \alpha p)$-lower-regular and $(V_2, V_3)$ is
%       $(\eps^\star, \alpha p)$-lower-regular in $G$, and
%     \item $|V_1|, |V_3| \geq \mu np$ and $|V_2| \geq \mu n$.
%   \end{itemize}
%   Then the set of vertices $v \in V_1$ satisfying
%   \[
%     |N_G(v, V_2)| \geq (1 - \eps)|V_2|\alpha p \qquad \text{and} \qquad \big(
%     N_G(v, V_2), V_3 \big) \text{ is $(\eps, \alpha p)$-lower-regular},
%   \]
%   is of size at least $(1 - \eps)|V_1|$.
% \end{proposition}

% It does not come as a big surprise that the inheritance is actually `two-sided'.
% Namely, if $(V_1, V_2)$, $(V_2, V_3)$, and $(V_1, V_3)$ are $(\eps, \alpha
% p)$-lower-regular in $\Gnp$, most of the vertices in $V_1$ are such that their
% neighbourhoods into $V_2$ and $V_3$ are also $(\eps', \alpha p)$-lower-regular.
% Perhaps the only important difference to the statement above is that the density
% $p$ of the random graph we are working with is such that the `two-sided'
% inheritance can only be shown to hold for linear-sized host sets. Similar
% statements (together with their proofs) to this one appeared in,
% e.g.~\cite{vskoric2018local, kohayakawa2011sparse, noever2017local}.

% \begin{proposition}\label{prop:two-sided-inheritance}
%   For all $\alpha, \eps, \mu > 0$, there exist positive constants
%   $\eps^\star(\alpha, \eps)$ and $C(\alpha, \eps)$ such that w.h.p.\ a random
%   graph $\Gamma \sim \Gnp$ satisfies the following, provided that $p \geq
%   Cn^{-2/5}$. Let $G \subseteq \Gamma$ and $V_1, V_2, V_3 \subseteq V(G)$ be
%   disjoint sets such that
%   \begin{itemize}
%     \item $(V_i, V_j)$ is $(\eps^\star, \alpha p)$-lower-regular for all $1 \leq
%       i < j \leq 3$, and
%     \item $|V_i| \geq \mu n$, for all $i \in [3]$.
%   \end{itemize}
%   Then the set of vertices $v \in V_1$ satisfying
%   \begin{itemize}
%     \item $|N_G(v, V_2)| \geq (1 - \eps)|V_2|\alpha p$ and $|N_G(v, V_3)| \geq
%       (1 - \eps)|V_3|\alpha p$, and
%     \item $\big( N_G(v, V_2), N_G(v, V_3) \big)$ is $(\eps, \alpha
%       p)$-lower-regular,
%   \end{itemize}
%   is of size at least $(1 - \eps)|V_1|$.
% \end{proposition}

% For us it turns out to be useful that not only neighbourhoods of a single vertex
% induce a regular pair, but that in certain sets almost all {\em pairs of
% vertices} have neighbourhoods which are regular with one another. A claim like
% this is perhaps slightly unnatural and thus, even though the proof follows
% standard methods (see, e.g.\ proof of Proposition~15
% in~\cite{kohayakawa2011sparse}), we prove it in (almost) full detail.

% \begin{proposition}\label{prop:double-inheritance}
%   For all $\alpha, \eps, \mu > 0$, there exist positive constants
%   $\eps'(\alpha)$, $\eps^\star(\alpha, \eps)$, and $C(\alpha, \eps, \mu)$ such
%   that w.h.p.\ a random graph $\Gamma \sim \Gnp$ satisfies the following,
%   provided that $p \geq Cn^{-2/5}$. Let $G \subseteq \Gamma$ and $V_1, V_2, V_3,
%   V_4 \subseteq V(G)$ be disjoint sets such that
%   \begin{itemize}
%     \item $(V_1, V_2)$ and $(V_3, V_4)$ are $(\eps', \alpha p)$-lower-regular,
%       $(V_2, V_3)$ is $(\eps^\star, \alpha p)$-lower-regular in $G$, and
%     \item $|V_1|, |V_4| \in \{\mu np, \mu n\}$ and $|V_2|, |V_3| = \mu n$.
%   \end{itemize}
%   Then there exist $V_1' \subseteq V_1$ and $V_4' \subseteq V_4$ of size $|V_1'|
%   \geq (1 - \eps)|V_1|$ and $|V_4'| \geq (1 - \eps)|V_4|$, such that for every
%   choice of $u \in V_1'$ and $v \in V_4'$, we have
%   \begin{itemize}
%     \item $|N_G(u, V_2)| \geq (1 - \eps)|V_2|\alpha p$ and $|N_G(v, V_3)| \geq
%       (1 - \eps)|V_3|\alpha p$, and
%     \item $\big( N_G(u, V_2), N_G(v, V_3) \big)$ is $(\eps, \alpha
%       p)$-lower-regular.
%   \end{itemize}
% \end{proposition}
% \begin{proof}
%   For clarity of presentation assume that $|V_1| = |V_4| = \mu np$. A proof
%   along the same lines works for the sets of different size as well, but is
%   tedious to present in a clean manner all at once. Let $\beta > 0$ be chosen to
%   satisfy $(2e/\alpha)^\alpha \cdot \beta^{\eps(1 - \eps)\alpha/2} < 1/e^2$, let
%   $\tilde\eps = \min{\{1/2,
%   \eps^\star_{\ref{lem:small-regularity-inheritance}}(\eps, \beta)\}}, \eps' =
%   \eps'_{\ref{prop:one-sided-inheritance}}(\alpha)$, and $\eps^\star =
%   \min{\{\eps/4, \eps^\star_{\ref{prop:one-sided-inheritance}}(\alpha,
%   \tilde\eps) \}}$. Take $C = \max{\{
%   C_{\ref{lem:small-regularity-inheritance}}(\eps),
%   C_{\ref{prop:one-sided-inheritance}}(\alpha, \tilde\eps, \mu) \}}$ and write
%   $s = \mu n$.

%   By Proposition~\ref{prop:one-sided-inheritance}, w.h.p.\ $\Gamma \sim \Gnp$ is
%   such that every $G \subseteq \Gamma$ as in the statement satisfies the
%   following. There is a set of vertices $V_1' \subseteq V_1$ which is of size at
%   least $(1 - \tilde\eps)|V_1|$ where
%   \[
%     |N_G(u, V_2)| \geq (1 - \tilde\eps)|V_2|\alpha p \quad \text{ and } \quad
%     (N_G(u, V_2), V_3) \text{ is $(\tilde\eps, \alpha p)$\text{-lower-regular}},
%   \]
%   for all $u \in V_1'$. From now on we condition on this event. For every such
%   $u \in V_1'$, let $N_u := N_G(u, V_2)$.

%   Let $\cB$ be the class of graphs obtained as follows. Every $G \in \cB$ has
%   $V_1' \cup V_2 \cup V_3 \cup V_4$ as a vertex set, with $(V_3, V_4)$ being
%   $(\eps', \alpha p)$-lower-regular and $(N_u, V_3)$ being $(\tilde\eps, \alpha
%   p)$-lower-regular for every $u \in V_1'$. Moreover, there is a set $X
%   \subseteq V_4$ of size $|X| > \eps sp$, such that for every $v \in X$ either
%   $|N_G(v, V_3)| < (1 - \eps)|V_3|\alpha p$ or there exists a $u \in V_1'$ for
%   which $(N_u, N_G(v, V_3))$ is not $(\eps, \alpha p)$-lower-regular. Let $Y
%   \subseteq X$ where every $v \in Y$ satisfies $|N_G(v, V_3)| \geq (1 -
%   \eps)|V_3|\alpha p$. Since $(V_3, V_4)$ is $(\eps', \alpha p)$-lower-regular,
%   it suffices to restrict $\cB$ only to those graphs for which $|Y| \geq
%   (\eps/2)sp$. We aim to show that $\cB$ is small enough in order for $\Gnp$ to
%   w.h.p.\ be such that none of $G \in \cB$ appear as its subgraph.

%   Without loss of generality we may assume $|Y| = (\eps/2)sp$. For $v \in Y$ let
%   $Y_v := N_G(v, V_3)$. Since $(N_u, Y_v)$ is not $(\eps, \alpha
%   p)$-lower-regular for a particular choice of $u$ and $v$, a straightforward
%   averaging argument shows that there exist sets $Y_v' \subseteq Y_v$ and $N_u'
%   \subseteq N_u$, each of size exactly $\eps(1 - \eps)s \alpha p$, such that
%   $d_G(N_u', Y_v') < (1 - \eps)\alpha p$. Let $Y_v''$ and $N_u''$ be sets of
%   size exactly $(1 - \eps)s\alpha p$ and such that $Y_v' \subseteq Y_v''
%   \subseteq Y_v$ and $N_u' \subseteq N_u'' \subseteq N_u$. Clearly, $(N_u'',
%   Y_v'')$ is not $(\eps, \alpha p)$-lower-regular. Therefore, for every $G \in
%   \cB$, there is a family of pairs $\{ (N_u'', Y_v'') : u \in V_1', v \in Y\}$
%   such that $(N_u'', Y_v'')$ is not $(\eps, \alpha p)$-lower-regular. We show
%   that such a configuration is unlikely to appear in $\Gnp$.

%   The number of choices for sets $V_1', V_2, V_3, Y$, vertices $u \in V_1'$,
%   and edges in the bipartite graph $(N_u'', V_3)$ which is $(\tilde\eps, \alpha
%   p)$-lower-regular is at most
%   \[
%     n \cdot \binom{n}{sp}^2 \cdot \binom{n}{s}^2 \cdot \sum_{m \geq (1 -
%     \tilde\eps)\alpha s^2p^2} \binom{s^2p}{m}.
%   \]
%   Next, for a fixed $v \in Y$, the number of configurations in which there is a
%   $u \in V_1'$ for which $(N_u'', Y_v'')$ does not form an $(\eps, \alpha
%   p)$-lower-regular pair is by Lemma~\ref{lem:small-regularity-inheritance} at
%   most
%   \[
%     s \cdot \beta^{(1 - \eps)\alpha sp} \binom{s}{(1 - \eps)\alpha sp}.
%   \]
%   As $|Y| = (\eps/2)sp$, the number of choices for such `bad' configurations is
%   bounded by
%   \[
%     \bigg( s \cdot \beta^{(1 - \eps)\alpha sp} \cdot \binom{s}{(1 - \eps)\alpha
%     sp} \bigg)^{(\eps/2)sp}.
%   \]
%   Therefore, the total number of graphs $G \in \cB$ is at most
%   \begin{align*}
%     |\cB| & \leq \sum_{m \geq (1 - \tilde\eps)\alpha s^2p^2} n \binom{n}{sp}^2
%     \binom{n}{s}^2 \binom{s^2p}{m} \cdot \bigg( s \cdot \beta^{(1 - \eps)\alpha
%     sp} \cdot \binom{s}{(1 - \eps)\alpha sp} \bigg)^{(\eps/2)sp} \\
%     %
%     & \leq \sum_{m \geq (1 - \tilde\eps)\alpha s^2p^2} e^{7n\log n} \binom{s^2
%     p}{m} \bigg( \beta^{(1 - \eps)\alpha sp} \cdot \binom{s}{(1 - \eps)\alpha
%     sp} \bigg)^{(\eps/2)sp}.
%   \end{align*}

%   It remains to show that w.h.p.\ none of these graphs appears as a subgraph of
%   $\Gnp$. The expected number of these graphs in $\Gnp$ is at most
%   \[
%     \sum_{m \geq (1 - \tilde\eps)\alpha s^2p^2} e^{7n\log n} \binom{s^2 p}{m}
%     p^m \cdot \bigg( \beta^{(1 - \eps)\alpha sp} \cdot \binom{s}{(1 -
%     \eps)\alpha sp} \bigg)^{(\eps/2)sp} p^{(\eps/2)sp \cdot (1 - \eps)\alpha
%     sp}.
%   \]
%   A routine calculation shows that the quantity above can be bounded by
%   \[
%     \sum_{m \geq (1 - \tilde\eps)\alpha s^2p^2} e^{7n\log n} \Big( \frac{e
%     s^2p^2}{m} \Big)^m \cdot \Big( \beta \frac{e}{(1 - \eps)\alpha} \Big)^{(1 -
%     \eps)(\eps/2)\alpha s^2p^2} \leq e^{9n\log n} \Big( e \cdot \Big(
%     \frac{2e}{\alpha} \Big)^\alpha \cdot \beta^{\eps(1 - \eps)\alpha/2}
%     \Big)^{s^2 p^2},
%   \]
%   where the last inequality follows from the fact that $(es^2p^2/m)^m$ is
%   maximised for $m = s^2p^2$. Since $\beta$ is chosen to satisfy
%   $(2e/\alpha)^\alpha \cdot \beta^{\eps(1 - \eps)\alpha/2} < 1/e^2$, we further
%   get that the expected number of such graph is at most
%   \[
%     e^{7n \log n} \cdot e^{-s^2p^2} = o(1),
%   \]
%   as $s^2 p^2 \geq (\mu n)^2 p^2 \geq C^2 \mu^2 n^{6/5} \gg n \log n$. By
%   Markov's inequality w.h.p.\ none of the graphs belonging to $\cB$ appears as a
%   subgraph of $\Gnp$ and the proof is complete.
% \end{proof}

% \subsection{Regularity inheritance: edge subsets}

% Similarly as is the case for taking/removing vertex subsets, removing a
% negligible fraction of the edges from the regular pair does not change the
% regularity parameter too much.

% \begin{proposition}\label{prop:edge-subset-reg-inheritance}
%   Let $\eps, p \in (0, 1)$, and let $(X, Y)$ be an $(\eps, p)$-regular pair in a
%   graph $G$. Let $G'$ be a graph obtained by removing at most $\eps^3|X||Y|p$
%   edges from $G[X, Y]$. Then $(X, Y)$ is $(3\eps, p)$-regular in $G'$.
% \end{proposition}

% \begin{proof}
%   Let $X' \subseteq X$ and $Y' \subseteq Y$ be subsets of size $|X'| \geq
%   3\eps|X|$ and $|Y'| \geq 3\eps|Y|$. Then
%   \[
%     |d_G(X', Y') - d_{G'}(X', Y')| \leq \frac{e_G(X', Y') - e_{G'}(X',
%     Y')}{|X'||Y'|} \leq \frac{\eps^3|X||Y|p}{\eps^2|X||Y|} \leq \eps p.
%   \]
%   The statement follows from triangle inequality.
% \end{proof}

% The other important property regarding the edges in $(\eps, p)$-regular
% subgraphs $(X, Y, Z)$ in a random graph $\Gnp$ is that most of the edges
% between, say $X$ and $Y$, are such that their endpoints have common neighbours
% in the set $Z$. This follows from the fact that most of the vertices in $X$ are
% `typical' with respect to $Y$ and $Z$ in the sense that their neighbourhoods are
% $(\eps', p)$-regular, giving rise to a plentiful of `typical' edges with common
% neighbours.

% \begin{proposition}\label{prop:typical-edges}
%   For every $\alpha, \eps', \xi > 0$, there exist positive constants
%   $\eps(\alpha, \eps', \xi)$ and $C(\alpha, \eps', \xi)$ such that w.h.p.\ a
%   random graph $\Gamma \sim \Gnp$ satisfies the following, provided that $p \geq
%   Cn^{-2/5}$. Let $G \subseteq \Gamma$ and $V_1, V_2, V_3 \subseteq V(G)$ be
%   such that
%   \begin{itemize}
%     \item $(V_1, V_2, V_3)$ is $(\eps, p)$-regular of density at least $\alpha
%       p$ in $G$, and
%     \item $|V_1|, |V_2|, |V_3| \geq \xi n$.
%   \end{itemize}
%   Then there are at most $4\eps' d_G(V_1, V_2) |V_1||V_2|$ edges in $G[V_1,
%   V_2]$ whose endpoints have no common neighbour in $V_3$.
% \end{proposition}
% \begin{proof}
%   Let $\eps$ be small enough depending on $\alpha$, $\eps'$, and $\xi$ such that
%   the arguments below go through. First, there are at least $(1 - \eps)|V_1|$
%   vertices $u \in V_1$ such that $|N_G(u, V_2)| = (1 \pm \eps) d_G(V_1, V_2)
%   |V_2|$, by definition of a regular pair. Furthermore, there are at least $(1 -
%   \eps')|V_1|$ vertices $u \in V_1$ such that $(N_G(u, V_2), N_G(u, V_3))$ is
%   $(\eps', \alpha p)$-lower-regular, by
%   Proposition~\ref{prop:two-sided-inheritance}. Therefore, as
%   \[
%     (1 - \eps')\alpha|N_G(v, V_2)|p \geq (1 - \eps')^2 \alpha^2 |V_2| p^2 > 0
%   \]
%   there are at least $(1 - \eps')|N_G(v, V_2)|$ vertices $v \in V_2$ which have
%   a neighbour in $N_G(u, V_3)$, making the edge $uv$ have a common neighbour in
%   $V_3$. Consequently, there are at most
%   \[
%     |V_1| \cdot \eps'|N_G(v, V_2)| \leq \eps' (1 + \eps) d_G(V_1, V_2)|V_1||V_2|
%     \leq 2\eps' d_G(V_1, V_2)|V_1||V_2|
%   \]
%   edges in $G[V_1, V_2]$ which are incident to `typical' vertices of $V_1$ and
%   whose endpoints do not have a common neighbour in $V_3$.

%   On the other hand, between the at most $\eps'|V_1|$ vertices which are not
%   `typical' and $V_2$ there are at most
%   \[
%     (d_G(V_1, V_2) + \eps p) \eps'|V_1||V_2| \leq 2\eps' d_G(V_1, V_2)
%     |V_1||V_2|
%   \]
%   edges, as $(V_1, V_2)$ is $(\eps, p)$-regular and $d_G(V_1, V_2) \geq \alpha
%   p$. This completes the proof.
% \end{proof}

% \subsection{K{\L}R conjecture and how to embed a cycle}

% Given a graph $H$ on $t \in \N$ vertices $\{1, \dotsc, t\}$, an integer $n$, and
% $\eps, p \in (0, 1)$, we let $\cG(H, n, \eps, p)$ denote the class of all graphs
% obtained as follows. The vertex set of $G \in \cG(H, n, \eps, p)$ is a disjoint
% union of sets $V_1 \cup \dotsb \cup V_t$, each of size $n$, and the edge set is
% given by an $(\eps, p)$-lower-regular pair $(V_i, V_j)$ for which $ij \in H$.
% Recall, a {\em canonical copy} of $H$ in $G$ is a $t$-tuple $(v_1, \dotsc, v_t)$
% such that $v_i \in V_i$ and $v_iv_j \in G$ for every $ij \in H$.

% The following is a statement which shows the existence of a graph $H$ in a
% member of the class $\cG(H, n, \eps, p)$ under certain conditions. The full
% version became known as the notorious {\em K{\L}R conjecture} and has since been
% converted into a theorem by Balogh, Morris, and
% Samotij~\cite{balogh2015independent} as well as, independently, Saxton and
% Thomasson~\cite{saxton2015hypergraph} via the method of hypergraph containers.
% (We refer an interested reader to~\cite{conlon2014klr} for more on
% K{\L}R, counting versions, numerous applications in extremal combinatorics,
% etc.) However, even before that major breakthrough, the conjecture had been
% known to hold for some `natural' classes of graphs, e.g.\ cycles and
% cliques~\cite{behrisch2002random, gerke2007small, gerke2007k}. For our purposes,
% such a `simpler version' would have been enough as we only ever apply it for $H$
% being either a cycle $C_\ell$ or $K_4$.
% % We state one such simple version tailored for random graphs that turns out to be
% % sufficient for our needs.

% \begin{proposition}[Sparse embedding lemma]
%   \label{thm:klr-random-graphs}
%   For every graph $H$ there exist positive constants $\eps$ and $D$ such that
%   for every integer $\tilde n \geq Dp^{-m_2(H)}$ a random graph $\Gamma \sim
%   \Gnp$ w.h.p.\ satisfies the following. Let $G \subseteq \Gamma$ belong to
%   $\cG(H, \tilde n, \eps, p)$. Then there is a canonical copy of $H$ in $G$.
% \end{proposition}

% Given $\ell \in \N$ and $\delta > 0$, we say that a graph $G = (V, E)$ is
% $(\delta, \ell)$-expanding for sets $S, T \subseteq V$ if for at least $(1 -
% \delta)|S|$ vertices $v \in S$ there are $(1 - \delta)|T|$ vertices of $T$ at
% distance at most $\ell$ from $v$. The next lemma is a reformulation of
% \cite[Lemma~5.6]{gerke2007small} suitable for applications in random graphs, and
% follows from it combined with a simple counting argument.

% \begin{lemma}\label{lem:regularity-expansion}
%   For every $\delta > 0$ there exist positive constants $\eps(\delta)$ and
%   $D(\delta)$ such that for every integer $\tilde n \geq Dp^{-3/2}$ w.h.p.\ a
%   random graph $\Gamma \sim \Gnp$ satisfies the following. Every $G \subseteq
%   \Gamma$ belonging to $\cG(P_4, n, \eps, p)$ is $(\delta, 3)$-expanding for
%   $V_1$ and $V_\ell$.
% \end{lemma}

% With a combination of several statements from above we are ready to present a
% short---but crucial---lemma used in the proof of our main result. It provides us
% the ability to, under certain conditions, embed cycles of any length into sets
% of size only roughly $np$.

% \begin{lemma}\label{lem:cycle-embedding-lemma}
%   For all $\alpha, \mu > 0$, there exist positive constants $\beta(\alpha,
%   \mu)$, $\eps(\alpha)$, and $C(\alpha, \mu)$ such that w.h.p.\ a random
%   graph $\Gamma \sim \Gnp$ satisfies the following, provided that $p \geq
%   Cn^{-2/5}$.

%   Let $4 \leq t \leq \beta n$, $G \subseteq \Gamma$, and let $\{s_1, \dotsc,
%   s_t\}$ be a subset of $V(G)$. Suppose $V_1, \dotsc, V_t \subseteq V(G)$ are
%   disjoint from $s_1, \dotsc, s_t$ such that:
%   \begin{enumerate}[(i)]
%     \item $V_i \subseteq N_G(s_i)$ and $|V_i| = \mu np$, for all $i \in [t]$,
%       and
%     \item $(V_t, V_1)$ and $(V_i, V_{i + 1})$ are $(\eps, \alpha
%       p)$-lower-regular in $G$, for all $i \in [t - 1]$.
%   \end{enumerate}

%   Then there is a canonical copy of a cycle $C_t$ in $G[V_1 \cup \dotsb \cup
%   V_t]$.
% \end{lemma}
% \begin{proof}
%   Write $\tilde n := \mu np/10$. Let $\beta =
%   \beta_{\ref{lem:tree-embedding-lemma}}(\alpha/2, \mu/40)$, $\eps' =
%   \min{\{
%       \eps_{\ref{thm:klr-random-graphs}}(C_4),
%       \eps_{\ref{lem:regularity-expansion}}(1/4)
%   \}}$,
%   $C = 10\mu^{-1} \cdot
%   \max{\{
%     C_{\ref{lem:tree-embedding-lemma}}(\alpha/2, \mu/40),
%     D_{\ref{thm:klr-random-graphs}}(C_4),
%     D_{\ref{lem:regularity-expansion}}(1/4)
%   \}}$, and $\eps =
%   \eps'/80$.

%   If $4 \leq t \leq 6$, for all $i \in [t]$ let $U_i \subseteq V_i$ be disjoint
%   subsets of size $|U_i| = \tilde n$. Then, by
%   Proposition~\ref{prop:large-subset-reg-inheritance} the graph $G[U_1 \cup
%   \dotsb \cup U_t]$ belongs to the class $\cG(C_t, \tilde n, 10\eps, \alpha p)$.
%   Therefore, as $m_2(C_4) > m_2(C_5) > m_2(C_6)$ and
%   \[
%     \tilde n = \mu np/10 \geq (\mu/10) \cdot Cp^{-5/2} \cdot p \geq
%     D_{\ref{thm:klr-random-graphs}}(C_4)p^{-3/2} =
%     D_{\ref{thm:klr-random-graphs}}(C_4)p^{-m_2(C_4)},
%   \]
%   Proposition~\ref{thm:klr-random-graphs} applied with $C_t$ (as $H$) shows the
%   existence of a canonical copy of $C_t$ in $G[V_1 \cup \dotsb \cup V_t]$ as
%   required.

%   If $t \geq 7$, the procedure is a bit more involved. First, let $U_i \subseteq
%   V_i$ be disjoint subsets of size $|U_i| = \tilde n$, for all $i \in [7]$.
%   Next, by Lemma~\ref{lem:regularity-expansion} for $\delta = 1/4$, as
%   \[
%     \tilde n = \mu np/10 \geq (\mu/10) \cdot Cp^{-5/2} \cdot p \geq
%     D_{\ref{lem:regularity-expansion}}(1/4)p^{-3/2},
%   \]
%   we get that there is a vertex $v \in U_4$ which is $(1/4, 3)$-expanding for
%   $U_7$ through $U_5, U_6$ and simultaneously $(1/4, 3)$-expanding for $U_1$
%   through $U_3, U_2$. Let $U_7' \subseteq U_7$ and $U_1' \subseteq U_1$ be of
%   size $\tilde n/2$ and such that $v$ expands to all vertices of $V_1'$ and
%   $V_5'$. Let $V_1' \subseteq U_1'$ be of size $\tilde n/4$ and observe that $v$
%   expands to all vertices of $V_1'$. For every $i = t, \dotsc, 8$, let $V_i'
%   \subseteq V_i$ and $V_7' \subseteq U_7'$ be subsets disjoint from $\bigcup_{2
%   \leq j \leq 6} U_j$ of size $|V_i'| = |V_7'| = \tilde n/4$ such that all $u
%   \in V_t'$ satisfy $\deg_G(u, V_1') \geq (\alpha/2)|V_1'|p$ and, for all $i <
%   t$, all $u \in V_i'$ satisfy $\deg_G(u, V_{i + 1}') \geq (\alpha/2)|V_{i +
%   1}'|p$. Such subsets can be chosen sequentially and greedily as $(V_t, V_1')$
%   and $(V_i, V_{i + 1}')$ are $(80\eps, \alpha p)$-lower-regular for all $7 \leq
%   i \leq t - 1$, by Proposition~\ref{prop:large-subset-reg-inheritance}.

%   We now apply Lemma~\ref{lem:tree-embedding-lemma} with $\alpha/2$ (as
%   $\alpha$), $\mu/40$ (as $\mu$), $t - 5$ (as $t$), and $V_7', \dotsc, V_t',
%   V_1'$ (as $V_1, \dotsc, V_t$) in order to find a canonical copy of $P_{t - 5}$
%   in $G[V_7' \cup \dotsb \cup V_t' \cup V_1']$ which starts at some vertex in
%   $V_7'$ and ends at some vertex in $V_1'$. Clearly, as $v$ expands to both
%   $V_1' \subseteq U_1'$ and $V_7' \subseteq U_7'$, and the path does not use any
%   vertices of $\bigcup_{2 \leq i \leq 6} U_i$, it closes a canonical copy of
%   $C_t$ in $G[V_1 \cup \dotsb \cup V_t]$.
% \end{proof}

